Privacy-Enhanced Database Synthesis for Benchmark Publishing (Technical Report)

Benchmarking is crucial for evaluating a DBMS, yet existing benchmarks often fail to reflect the varied nature of user workloads. As a result, there is increasing momentum toward creating databases that incorporate real-world user data to more accurately mirror business environments. However, privacy concerns deter users from directly sharing their data, underscoring the importance of creating synthesized databases for benchmarking that also prioritize privacy protection. Differential privacy (DP)-based data synthesis has become a key method for safeguarding privacy when sharing data, but the focus has largely been on minimizing errors in aggregate queries or downstream ML tasks, with less attention given to benchmarking factors like query runtime performance. This paper delves into differentially private database synthesis specifically for benchmark publishing scenarios, aiming to produce a synthetic database whose benchmarking factors closely resemble those of the original data. Introducing \textit{PrivBench}, an innovative synthesis framework based on sum-product networks (SPNs), we support the synthesis of high-quality benchmark databases that maintain fidelity in both data distribution and query runtime performance while preserving privacy. We validate that PrivBench can ensure database-level DP even when generating multi-relation databases with complex reference relationships. Our extensive experiments show that PrivBench efficiently synthesizes data that maintains privacy and excels in both data distribution similarity and query runtime similarity.

==> alg.tex <==
\appendix

\begin{algorithm} [ht]
  \caption{Private SPN Construction \kw{PrivSPN} (Beta 0)}
  \SetKwComment{tcp}{//}{}
  \Input{table $T$, total privacy budget $\epsilon$. } 
  \Output{A tree of SPN $t=(\kw{parent}, \kw{left}, \kw{right})$, privacy loss $\epsilon_t$ for tree construction}
  \KwParam{privacy budgets $\epsilon_v$ (validation), $\epsilon_c$ (column splitting), $\epsilon_r$ (row splitting), $\epsilon_h$ (leaf node)}
  \SetKwProg{Procedure}{procedure}{}{}
  \Procedure{\kw{PrivSPN}($T, \epsilon$)}{
  \Return{\kw{recursiveSplit}($T, \epsilon$)\;}
  }
  \Procedure{\kw{recursiveSplit}($T, \bar{\epsilon}$)}{
    % \tcp*[h]{op is the next splitting operation}\;
    $\kw{op}\leftarrow \kw{planning}(T, \bar{\epsilon})$, $\epsilon_{t} \leftarrow \epsilon_v$\;
    \If{$\kw{op} = \kw{OP}.\kw{CREATELEAF}$}{
        \Return{\kw{LeafNode}($T, \epsilon_h$), $\epsilon_h$}
    }    
    \ElseIf{$\kw{op} = \kw{OP}.\kw{SPLITROWS}$}{
        $(\widetilde{S}_L, \widetilde{S}_R) \leftarrow \kw{splitRowsWithClustering}(T, \epsilon_r)$,
        $\epsilon_{t} \leftarrow \epsilon_{t} + \epsilon_{r}$, $\kw{parent} \leftarrow \kw{SumNode}$\;
    } 
    \ElseIf{$\kw{op} = \kw{OP}.\kw{RNDCUTROWS}$}{$(\widetilde{S}_L, \widetilde{S}_R) \leftarrow \kw{randomCutRows}(T)$, $\kw{parent} \leftarrow \kw{SumNode}$\;} 
    \ElseIf{$\kw{op} = \kw{OP}.\kw{SPLITCOLS}$}{
    $(\widetilde{S}_L, \widetilde{S}_R) \leftarrow \kw{columnSplit} (T, \epsilon_c)$, $\epsilon_{t} \leftarrow \epsilon_{t} + \epsilon_{c}$, $\kw{parent} \leftarrow \kw{ProductNode}$\;            
    }
    \ElseIf{$\kw{op} = \kw{OP}.\kw{RNDSPLITCOLS}$}{$(\widetilde{S}_L, \widetilde{S}_R) \leftarrow \kw{randomSplitCols}(T)$, $\kw{parent} \leftarrow \kw{ProductNode}$}
    $T_{L} \leftarrow T[\widetilde{S}_L], T_{R} \leftarrow T[\widetilde{S}_R]$\; 
    $\kw{left}, \epsilon_{\kw{left}} \leftarrow \kw{recursiveSplit}(T_{L}, \bar{\epsilon} - \epsilon_t)$\;
    $\kw{right}, \epsilon_{\kw{right}} \leftarrow \kw{recursiveSplit}(T_{R}, \bar{\epsilon} - \epsilon_t - \epsilon_{\kw{left}})$\;
    \If{$\kw{op} = \kw{OP}.\kw{SPLITROWS} | \kw{OP}.\kw{RNDCUTROWS}$}{
        $\epsilon_{t} \leftarrow \epsilon_t + \max\{\epsilon_{\kw{left}}, \epsilon_{\kw{right}}\}$
    }
    \Else{$\epsilon_{t} \leftarrow \epsilon_t + \epsilon_{\kw{left}} + \epsilon_{\kw{right}}$}
    \Return{$(\kw{parent}, \kw{left}, \kw{right})$, $\epsilon_{t}$}\;
    
    % \If{$op = OP.SPLIT\_COLS$}{
    %     $(\textbf{a}_l, \textbf{a}_r, isFail ) \leftarrow split\_cols(T, \textbf{a}, \alpha, force)$\;
    %     $lch \leftarrow splitDatabase(\textbf{a}_l, \textbf{r}, T)$\;
    %     $rch \leftarrow splitDatabase(\textbf{a}_r, \textbf{r}, T)$\;
    %     \Return ProductNode($lch, rch, \textbf{a}, \textbf{r}$)
    % }  
}
\end{algorithm}
 
\begin{algorithm} [ht]
    \caption{Planning Next Operation \kw{planning} (Beta 0)}
    \Input{table $T$, privacy budget $\bar{\epsilon}$}
    \Output{next operation $op$}
    \KwParam{privacy budgets $\epsilon_c$ (column splitting), $\epsilon_r$ (row splitting), $\epsilon_v$ (validation), $\epsilon_h$ (leaf node), thresholds $\alpha$ (column splitting), $\beta$ (row splitting)}
    \SetKwProg{Procedure}{procedure}{}{}
        \Procedure{\kw{planning}($ T, \bar{\epsilon}$)}{
        % \If{$|T.\kw{Attributes}| = 1$}{
        %     \If{$|T| > \beta$}{     
        %         \If{$\bar{\epsilon} \geq \epsilon_r$}
        %             {\Return\ \kw{OP}.\kw{SPLITROWS}}
        %         \Else
        %             {\Return\ \kw{OP}.\kw{RNDCUTROWS}}
        %     }
        %     \Return\ \kw{OP}.\kw{CREATELEAF}
        % }
        \If{\kw{validateColumnSplit}($T$)}{
            \If{$\bar{\epsilon} \geq \epsilon_c + \epsilon_h$}{
                \Return\ \kw{OP}.\kw{SPLITCOLS}\;
            }
            \Else{
                \Return\ \kw{OP}.\kw{RNDSPLITCOLS}\;
            }
    
        }
        \Else{
            \If{$|T| > \beta$}{  
                \If{$\bar{\epsilon} \geq \epsilon_r + \epsilon_h$}
                    {\Return\ \kw{OP}.\kw{SPLITROWS}}
                \Else
                    {\Return\ \kw{OP}.\kw{RNDCUTROWS}}
            }
            \ElseIf{$|T.\kw{Attributes}| > 1$}{\Return\ \kw{OP}.\kw{RNDSPLITCOLS}}
            \Return\ \kw{OP}.\kw{CREATELEAF}\;
        }
        }
    \Procedure{\kw{validateColumnSplit}($T$)}{
        \If{$|T.\kw{Attributes}| = 1$}{\Return $\kw{False}$\;}
        % $\mathcal{S} \leftarrow T.\kw{Attributes}$, ${MIList} \leftarrow \emptyset$\;
        % \For{each binary partition $(\mathcal{S}_L,\mathcal{S}_R)$ of $\mathcal{S}$}
        %     {Add $MI(T[\mathcal{S}_L], T[\mathcal{S}_L])$ into $MIList$;}
        % ${minMI} \leftarrow \min_{\mathcal{S}_L, \mathcal{S}_R} MI(T[\mathcal{S}_L], T[\mathcal{S}_R])$\;
        % $q(T_{param}, \widetilde{\mathcal{S}_L},\widetilde{\mathcal{S}_R}) = MI(T_{param}[\widetilde{\mathcal{S}_L}], T_{param}[\widetilde{\mathcal{S}_R}]) - {minMI}$\;
        % $\Delta q = \max_{\mathcal{S}_L, \mathcal{S}_R, T_{param}} MI(T_{param}[\mathcal{A_L}], T_{param}[\mathcal{A_R}])$\;
        % Sample partition $(\widetilde{\mathcal{S}_L},\widetilde{\mathcal{S}_R})$ with probability $exp(\frac{-\epsilon_v \cdot q(T, \widetilde{\mathcal{S}_L},\widetilde{\mathcal{S}_R})}{2\Delta q})$\;
        $\widetilde{\mathcal{S}}_L, \widetilde{\mathcal{S}}_R \leftarrow \kw{columnSplit(T, \epsilon_v)}$\;
        \If{$MI(T[\widetilde{\mathcal{S}}_L], T[\widetilde{\mathcal{S}}_R]) + \kw{Lap}(\frac{\Delta(NMI)}{\epsilon_v}) > \alpha$}
            {\Return $\kw{False}$\;}
        \Return $\kw{True}$\;
    }

\end{algorithm}

\clearpage
\begin{algorithm} [ht]
  \caption{Private SPN Construction \kw{PrivSPN} (Beta 1)}
  % \label{alg:SPN}
  \SetKwComment{tcp}{//}{}
  \Input{table $T$, total privacy budget $\epsilon$. } 
  \Output{A tree of SPN $t=(\kw{parent}, \kw{left}, \kw{right})$}
  \SetKwProg{Procedure}{procedure}{}{}
  \Procedure{$\kw{PrivSPN}(T, \epsilon)$}{
    % \tcp*[h]{op is the next splitting operation}\;
    $\kw{op}, \epsilon_p, \bar{\epsilon} \leftarrow \kw{planning}(T, \epsilon)$\;
    \If{$\kw{op} = \kw{OP}.\kw{CREATELEAF}$}{
        \Return{\kw{LeafNode}($T, \epsilon_p$)}
    }    
    \ElseIf{$\kw{op} = \kw{OP}.\kw{SPLITROWS}$}{
        $(\widetilde{S}_L, \widetilde{S}_R) \leftarrow \kw{splitRowsWithClustering}(T, \epsilon_p)$\;
        $\kw{parent} \leftarrow \kw{SumNode}(\widetilde{S}_L, \widetilde{S}_R)$\;
        $\epsilon_l \leftarrow \bar{\epsilon}, \epsilon_r \leftarrow \bar{\epsilon}$
    } 
    \ElseIf{$\kw{op} = \kw{OP}.\kw{SPLITCOLS}$}{
        $(\widetilde{S}_L, \widetilde{S}_R) \leftarrow \kw{columnSplit}(T, \epsilon_p)$\;
        $\kw{parent} \leftarrow \kw{ProductNode}(\widetilde{S}_L, \widetilde{S}_R)$\;
        $\epsilon_l \leftarrow \bar{\epsilon} \cdot \frac{\sigma(T[\widetilde{S}_L])}{\sigma(T[\widetilde{S}_L]) + \sigma(T[\widetilde{S}_R])}, \epsilon_r \leftarrow \bar{\epsilon} - \epsilon_l$
    }
    $\kw{left} \leftarrow \kw{recursiveSplit}(T[\widetilde{S}_L], \epsilon_{l})$\;
    $\kw{right} \leftarrow \kw{recursiveSplit}(T[\widetilde{S}_R], \epsilon_r)$\;
    \Return{$(\kw{parent}, \kw{left}, \kw{right})$}
    
    % \If{$op = OP.SPLIT\_COLS$}{
    %     $(\textbf{a}_l, \textbf{a}_r, isFail ) \leftarrow split\_cols(T, \textbf{a}, \alpha, force)$\;
    %     $lch \leftarrow splitDatabase(\textbf{a}_l, \textbf{r}, T)$\;
    %     $rch \leftarrow splitDatabase(\textbf{a}_r, \textbf{r}, T)$\;
    %     \Return ProductNode($lch, rch, \textbf{a}, \textbf{r}$)
    % }  
}
\end{algorithm}


\begin{algorithm} [ht]
    \caption{Operation Planning \kw{planning} (Beta 1)}
    % \label{alg:plan}
    \Input{table $T$, privacy budget $\epsilon$}
    \Output{next operation $\kw{op}$, privacy budget $\epsilon_p$ for $\kw{op}$, remaining privacy budget $\bar{\epsilon}$}
    \KwParam{buget ratio $\alpha$, minimum table size $\beta$}
    \SetKwProg{Procedure}{procedure}{}{}
        \Procedure{$\kw{planning}(T, \epsilon)$}{
            \If{$|T| < 2\beta$ and $|T.\kw{Attributes}| = 1$}{
                \Return\ \kw{OP}.\kw{CREATELEAF}, $(\epsilon, 0, 0)$
            }
            % \If{$|T| < 2\beta$ and $|T.\kw{Attributes}| = 2$}{
            %     \Return\ \kw{OP}.\kw{SPLITROWS}, $(0, \frac{\epsilon}{2}, \frac{\epsilon}{2})$
            % }
            $\bar{\epsilon}, \delta_{col}, \delta'_{col}, \delta_{row}, \delta'_{row} \leftarrow \kw{evalCorr}(T, \epsilon)$\;
            $\kw{op} \leftarrow \kw{decideOP}(T, \delta_{col}, \delta_{row})$\;
            $\epsilon_p, \bar{\epsilon} \leftarrow \kw{allocBudgetOP}(\kw{op}, \bar{\epsilon}, \delta_{col}, \delta_{row}))$\;
            \Return\ $\kw{op}, \epsilon_p, \bar{\epsilon}$
        }
        \Procedure{$\kw{evalCorr}(T, \epsilon)$}{
            $\epsilon_{eval} \leftarrow \alpha\cdot \epsilon, \delta_{col} \leftarrow 0, \delta_{row} \leftarrow 0$\;
            \If{$|T.\kw{Attributes}| > 1$}{
                % $(\mathcal{S}_L, \mathcal{S}_R) \leftarrow \kw{columnSplit}(T, \epsilon_{eval})$\;
                $(\mathcal{S}_L, \mathcal{S}_R) \leftarrow$ Sample the best column partition\;
                $(\mathcal{S}'_L, \mathcal{S}'_R) \leftarrow$ Sample the worst column partition\;
                $\delta_{col} \leftarrow \kw{NMI}_{col}(T[\mathcal{S}_L], T[\mathcal{S}_R]) + \kw{Lap}(\frac{\Delta(\kw{NMI}_{col})}{\epsilon_{eval}})$\;
                $\delta_{col}' \leftarrow \kw{NMI}_{col}(T[\mathcal{S}'_L], T[\mathcal{S}'_R]) + \kw{Lap}(\frac{\Delta(\kw{NMI}_{col})}{\epsilon_{eval}})$\;
                $\delta_{col} \leftarrow 2\cdot \kw{clip}(\delta_{col}, \kw{min}=0, \kw{max}=1)$\;
                $\delta_{col}' \leftarrow 2\cdot \kw{clip}(\delta'_{col}, \kw{min}=0, \kw{max}=1)$\;
                $\epsilon \leftarrow \epsilon - 2\epsilon_{eval}$
            }
            \If{$|T| \geq 2\beta$}{
                % $(\mathcal{S}_L, \mathcal{S}_R) \leftarrow \kw{splitRowsWithClustering}(T, \epsilon_{eval})$\;
                % $\delta_{row} \leftarrow \kw{NMI}_{row}(T[\mathcal{S}_L], T[\mathcal{S}_R]) + \kw{Lap}(\frac{\Delta(\kw{NMI}_{row})}{\epsilon_{eval}})$\;
                $(\mathcal{S}_L, \mathcal{S}_R) \leftarrow$ Sample the best row partition\;
                $(\mathcal{S}'_L, \mathcal{S}'_R) \leftarrow$ Sample the worst row partition\;
                $\delta_{row} \leftarrow \kw{NMI}_{row}(T[\mathcal{S}_L], T[\mathcal{S}_R]) + \kw{Lap}(\frac{\Delta(\kw{NMI}_{row})}{\epsilon_{eval}})$\;
                $\delta'_{row} \leftarrow \kw{NMI}_{row}(T[\mathcal{S}'_L], T[\mathcal{S}'_R]) + \kw{Lap}(\frac{\Delta(\kw{NMI}_{row})}{\epsilon_{eval}})$\;
                $\delta_{row} \leftarrow 2\cdot \kw{clip}(\delta_{row}, \kw{min}=0, \kw{max}=1)$\;
                $\delta'_{row} \leftarrow 2\cdot \kw{clip}(\delta'_{row}, \kw{min}=0, \kw{max}=1)$\;
                $\epsilon \leftarrow \epsilon - 2\epsilon_{eval}$
            }
            \Return\ $\epsilon, \delta_{col}, \delta'_{col}, \delta_{row}, \delta'_{row}$
        }
        \Procedure{$\kw{decideOP}(T, \delta_{col}, \delta_{row})$}{
            \If{$|T| \geq 2\beta$ and $|T.\kw{Attributes}| > 1$}{
                \If{$\delta_{col} < \delta_{row}$}{
                    $\kw{op} \leftarrow \kw{OP}.\kw{SPLITCOLS}$
                }
                \Else{
                    $\kw{op} \leftarrow \kw{OP}.\kw{SPLITROWS}$
                }
            }
            \ElseIf{$|T| \geq 2\beta$ and $|T.\kw{Attributes}| = 1$}{
                $\kw{op} \leftarrow \kw{OP}.\kw{SPLITROWS}$
            }
            \ElseIf{$|T| < 2\beta$ and $|T.\kw{Attributes}| > 1$}{
                $\kw{op} \leftarrow \kw{OP}.\kw{SPLITCOLS}$
            }
            \Return{\kw{op}}
        }
        \Procedure{$\kw{allocBudgetOP}(\kw{op}, \epsilon, \delta_{col}, \delta'_{col}, \delta_{row}, \delta'_{row})$}{
            \If{\kw{op} = \kw{OP}.\kw{SPLITROWS}}{
                $\epsilon_{p} \leftarrow \frac{(2 - |\delta_{row}-\delta'_{row}|) \cdot \epsilon}{\sigma(T)}$\;
            }
            \ElseIf{\kw{op} = \kw{OP}.\kw{SPLITCOLS}}{
                \If{$|T.\kw{Attributes}| = 2$}{
                    $\epsilon_{p} \leftarrow 0$\;
                }
                \Else{
                    $\epsilon_{p} \leftarrow \frac{(2-|\delta_{col}-\delta'_{col}|) \cdot \epsilon}{\sigma(T)}$\;
                }
            }
            \Return{$\epsilon_p, \epsilon - \epsilon_p$}
        }
\end{algorithm}


\begin{align*}
    \sigma(T) = 2\cdot |T.\kw{Attributes}| + \frac{|T|}{\beta} - 2
\end{align*}


\begin{align*}
    \kw{NMI}_{col}  = \big(\frac{2}{|T|}\log(\frac{|T|+1}{2}) + \frac{|T|-1}{|T|}\log(\frac{|T|+1}{|T|-1})\big) / \log(|T|)
\end{align*}

\begin{align*}
    \kw{NMI}_{row}  = & \big(\frac{\log(|T|)}{|T|} - \frac{|T|-1}{|T|}\log(\frac{|T|-1}{|T|})\\ 
    & + \frac{\log(n')}{n'} - \frac{n'-1}{n'}\log(\frac{n'-1}{n'})\big)/(\frac{\log(|T|) + \log(n')}{2})
\end{align*}
where $n'=\max\{|T[\mathcal{S}_L]|, |T[\mathcal{S}_R]|\}$


\clearpage

\begin{algorithm} [ht]
  \caption{Private SPN Construction \kw{PrivSPN} (Beta 2)}
  % \label{alg:SPN}
  \SetKwComment{tcp}{//}{}
  \Input{table $T$, total privacy budget $\epsilon$. } 
  \Output{A tree of SPN $t=(\kw{parent}, \kw{left}, \kw{right})$}
  \SetKwProg{Procedure}{procedure}{}{}
  \Procedure{$\kw{PrivSPN}(T, \epsilon)$}{
    % \tcp*[h]{op is the next splitting operation}\;
    $\kw{op}, \epsilon_p, \bar{\epsilon} \leftarrow \kw{planning}(T, \epsilon)$\;
    \If{$\kw{op} = \kw{OP}.\kw{CREATELEAF}$}{
        \Return{\kw{LeafNode}($T, \epsilon_p$)}
    }    
    \ElseIf{$\kw{op} = \kw{OP}.\kw{SPLITROWS}$}{
        $(\widetilde{S}_L, \widetilde{S}_R) \leftarrow \kw{splitRowsWithClustering}(T, \epsilon_p)$\;
        $\kw{parent} \leftarrow \kw{SumNode}(\widetilde{S}_L, \widetilde{S}_R)$\;
        $\epsilon_l \leftarrow \bar{\epsilon}, \epsilon_r \leftarrow \bar{\epsilon}$
    } 
    \ElseIf{$\kw{op} = \kw{OP}.\kw{SPLITCOLS}$}{
        $(\widetilde{S}_L, \widetilde{S}_R) \leftarrow \kw{columnSplit}(T, \epsilon_p)$\;
        $\kw{parent} \leftarrow \kw{ProductNode}(\widetilde{S}_L, \widetilde{S}_R)$\;
        $\epsilon_l \leftarrow \bar{\epsilon} \cdot \frac{\sigma(T[\widetilde{S}_L])}{\sigma(T[\widetilde{S}_L]) + \sigma(T[\widetilde{S}_R])}, \epsilon_r \leftarrow \bar{\epsilon} - \epsilon_l$
    }
    $\kw{left} \leftarrow \kw{recursiveSplit}(T[\widetilde{S}_L], \epsilon_{l})$\;
    $\kw{right} \leftarrow \kw{recursiveSplit}(T[\widetilde{S}_R], \epsilon_r)$\;
    \Return{$(\kw{parent}, \kw{left}, \kw{right})$}
    
    % \If{$op = OP.SPLIT\_COLS$}{
    %     $(\textbf{a}_l, \textbf{a}_r, isFail ) \leftarrow split\_cols(T, \textbf{a}, \alpha, force)$\;
    %     $lch \leftarrow splitDatabase(\textbf{a}_l, \textbf{r}, T)$\;
    %     $rch \leftarrow splitDatabase(\textbf{a}_r, \textbf{r}, T)$\;
    %     \Return ProductNode($lch, rch, \textbf{a}, \textbf{r}$)
    % }  
}
\end{algorithm}

\begin{algorithm}
    \caption{Operation Planning \kw{planning} (Beta 2)}
    % \label{alg:plan}
    \Input{table $T$, privacy budget $\epsilon$}
    \Output{next operation $\kw{op}$, privacy budget $\epsilon_p$ for $\kw{op}$, remaining privacy budget $\bar{\epsilon}$}
    \KwParam{threshold for column splitting $\alpha$, minimum table size $\beta$, budget ratios $\gamma_1, \gamma_2$}
    \SetKwProg{Procedure}{procedure}{}{}
        \Procedure{$\kw{planning}(T, \epsilon)$}{
            \If{$|T| < 2\beta$ and $|T.\kw{Attributes}| = 1$}{
                \Return\ \kw{OP}.\kw{CREATELEAF}, $(\epsilon, 0, 0)$
            }
            % \If{$|T| < 2\beta$ and $|T.\kw{Attributes}| = 2$}{
            %     \Return\ \kw{OP}.\kw{SPLITROWS}, $(0, \frac{\epsilon}{2}, \frac{\epsilon}{2})$
            % }
            $\bar{\epsilon}, \delta_{col} \leftarrow \kw{evalCorr}(T, \epsilon)$\;
            $\kw{op} \leftarrow \kw{decideOP}(T, \delta_{col})$\;
            $\epsilon_p, \bar{\epsilon} \leftarrow \kw{allocBudgetOP}(T, \kw{op}, \bar{\epsilon}))$\;
            \Return\ $\kw{op}, \epsilon_p, \bar{\epsilon}$
        }
        \Procedure{$\kw{evalCorr}(T, \epsilon)$}{
            $\epsilon_{eval} \leftarrow \gamma_1 \cdot \epsilon$\;
            \If{$|T.\kw{Attributes}| > 1$}{
                $(\mathcal{S}_L, \mathcal{S}_R) \leftarrow \kw{columnSplit}(T, \epsilon_{eval}\cdot \gamma_2)$\;
                $\delta_{col} \leftarrow \kw{NMI}_{col}(T[\mathcal{S}_L], T[\mathcal{S}_R]) + \kw{Lap}(\frac{\Delta(\kw{NMI}_{col})}{\epsilon_{eval}\cdot (1-\gamma_2)})$\;
                $\epsilon \leftarrow \epsilon -\epsilon_{eval}$
            }
            \Return\ $\epsilon, \delta_{col}$
        }
        \Procedure{$\kw{decideOP}(T, \delta_{col})$}{
            \If{$|T| \geq 2\beta$ and $|T.\kw{Attributes}| > 1$}{
                \If{$\delta_{col} \leq \alpha$}{
                    $\kw{op} \leftarrow \kw{OP}.\kw{SPLITCOLS}$
                }
                \Else{
                    $\kw{op} \leftarrow \kw{OP}.\kw{SPLITROWS}$
                }
            }
            \ElseIf{$|T| \geq 2\beta$ and $|T.\kw{Attributes}| = 1$}{
                $\kw{op} \leftarrow \kw{OP}.\kw{SPLITROWS}$
            }
            \ElseIf{$|T| < 2\beta$ and $|T.\kw{Attributes}| > 1$}{
                $\kw{op} \leftarrow \kw{OP}.\kw{SPLITCOLS}$
            }
            \Return{\kw{op}}
        }
        \Procedure{$\kw{allocBudgetOP}(T, \kw{op}, \epsilon)$}{
            \If{\kw{op} = \kw{OP}.\kw{SPLITCOLS} and $|T.\kw{Attributes}| = 2$}{
                $\epsilon_{p} \leftarrow 0$\;
            }
            \Else{
                $\epsilon_{p} \leftarrow \epsilon/\sigma(T)$\;
            }
       
            \Return{$\epsilon_p, \epsilon - \epsilon_p$}
        }
\end{algorithm}

\begin{align*}
    \sigma(T) = 2\cdot |T.\kw{Attributes}| + \frac{|T|}{\beta} - 2
\end{align*}


\begin{align*}
    \kw{NMI}_{col}  = \big(\frac{2}{|T|}\log(\frac{|T|+1}{2}) + \frac{|T|-1}{|T|}\log(\frac{|T|+1}{|T|-1})\big) / \log(|T|)
\end{align*}

\begin{align*}
    \kw{NMI}_{row}  = & \big(\frac{\log(|T|)}{|T|} - \frac{|T|-1}{|T|}\log(\frac{|T|-1}{|T|})\\ 
    & + \frac{\log(n')}{n'} - \frac{n'-1}{n'}\log(\frac{n'-1}{n'})\big)/(\frac{\log(|T|) + \log(n')}{2})
\end{align*}
where $n'=\max\{|T[\mathcal{S}_L]|, |T[\mathcal{S}_R]|\}$



\clearpage

\begin{algorithm} [ht]
  \caption{Private SPN Construction \kw{PrivSPN} (Beta 3)}
  % \label{alg:SPN}
  \SetKwComment{tcp}{//}{}
  \Input{table $T$, total privacy budget $\epsilon$. } 
  \Output{A tree of SPN $t=(\kw{parent}, \kw{left}, \kw{right})$}
  \SetKwProg{Procedure}{procedure}{}{}
  \Procedure{$\kw{PrivSPN}(T, \epsilon)$}{
    % \tcp*[h]{op is the next splitting operation}\;
    $\kw{op}, \epsilon_p, \bar{\epsilon} \leftarrow \kw{planning}(T, \epsilon)$\;
    \If{$\kw{op} = \kw{OP}.\kw{CREATELEAF}$}{
        \Return{\kw{LeafNode}($T, \epsilon_p$)}
    }    
    \ElseIf{$\kw{op} = \kw{OP}.\kw{SPLITROWS}$}{
        $(\widetilde{S}_L, \widetilde{S}_R) \leftarrow \kw{splitRowsWithClustering}(T, \epsilon_p)$\;
        $\kw{parent} \leftarrow \kw{SumNode}(\widetilde{S}_L, \widetilde{S}_R)$\;
        $\epsilon_l \leftarrow \bar{\epsilon}, \epsilon_r \leftarrow \bar{\epsilon}$
    } 
    \ElseIf{$\kw{op} = \kw{OP}.\kw{SPLITCOLS}$}{
        $(\widetilde{S}_L, \widetilde{S}_R) \leftarrow \kw{columnSplit}(T, \epsilon_p)$\;
        $\kw{parent} \leftarrow \kw{ProductNode}(\widetilde{S}_L, \widetilde{S}_R)$\;
        $\epsilon_l \leftarrow \bar{\epsilon} \cdot \frac{\sigma(T[\widetilde{S}_L])}{\sigma(T[\widetilde{S}_L]) + \sigma(T[\widetilde{S}_R])}, \epsilon_r \leftarrow \bar{\epsilon} - \epsilon_l$
    }
    $\kw{left} \leftarrow \kw{recursiveSplit}(T[\widetilde{S}_L], \epsilon_{l})$\;
    $\kw{right} \leftarrow \kw{recursiveSplit}(T[\widetilde{S}_R], \epsilon_r)$\;
    \Return{$(\kw{parent}, \kw{left}, \kw{right})$}
    
    % \If{$op = OP.SPLIT\_COLS$}{
    %     $(\textbf{a}_l, \textbf{a}_r, isFail ) \leftarrow split\_cols(T, \textbf{a}, \alpha, force)$\;
    %     $lch \leftarrow splitDatabase(\textbf{a}_l, \textbf{r}, T)$\;
    %     $rch \leftarrow splitDatabase(\textbf{a}_r, \textbf{r}, T)$\;
    %     \Return ProductNode($lch, rch, \textbf{a}, \textbf{r}$)
    % }  
}
\end{algorithm}

\begin{algorithm}
    \caption{Operation Planning \kw{planning} (Beta 3)}
    % \label{alg:plan}
    \Input{table $T$, privacy budget $\epsilon$}
    \Output{next operation $\kw{op}$, privacy budget $\epsilon_p$ for $\kw{op}$, remaining privacy budget $\bar{\epsilon}$}
    \KwParam{threshold for column splitting $\alpha$, minimum table size $\beta$, budget ratios $\gamma_1, \gamma_2$}
    \SetKwProg{Procedure}{procedure}{}{}
        \Procedure{$\kw{planning}(T, \epsilon)$}{
            \If{$|T| < 2\beta$ and $|T.\kw{Attributes}| = 1$}{
                \Return\ \kw{OP}.\kw{CREATELEAF}, $(\epsilon, 0, 0)$
            }
            % \If{$|T| < 2\beta$ and $|T.\kw{Attributes}| = 2$}{
            %     \Return\ \kw{OP}.\kw{SPLITROWS}, $(0, \frac{\epsilon}{2}, \frac{\epsilon}{2})$
            % }
            $\bar{\epsilon}, \delta_{col} \leftarrow \kw{evalCorr}(T, \epsilon)$\;
            $\kw{op} \leftarrow \kw{decideOP}(T, \delta_{col})$\;
            $\epsilon_p, \bar{\epsilon} \leftarrow \kw{allocBudgetOP}(T, \kw{op}, \bar{\epsilon}))$\;
            \Return\ $\kw{op}, \epsilon_p, \bar{\epsilon}$
        }
        \Procedure{$\kw{evalCorr}(T, \epsilon)$}{
            $\epsilon_{eval} \leftarrow \gamma_1 \cdot \epsilon$\;
            \If{$|T.\kw{Attributes}| > 1$}{
                $(\mathcal{S}_L, \mathcal{S}_R) \leftarrow \kw{columnSplit}(T, \epsilon_{eval}\cdot \gamma_2)$\;
                $\delta_{col} \leftarrow \kw{NMI}_{col}(T[\mathcal{S}_L], T[\mathcal{S}_R]) + \kw{Lap}(\frac{\Delta(\kw{NMI}_{col})}{\epsilon_{eval}\cdot (1-\gamma_2)})$\;
                $\epsilon \leftarrow \epsilon -\epsilon_{eval}$
            }
            \Return\ $\epsilon, \delta_{col}$
        }
        \Procedure{$\kw{decideOP}(T, \delta_{col})$}{
            \If{$|T| \geq 2\beta$ and $|T.\kw{Attributes}| > 1$}{
                \If{$\delta_{col} \leq \alpha$}{
                    $\kw{op} \leftarrow \kw{OP}.\kw{SPLITCOLS}$
                }
                \Else{
                    $\kw{op} \leftarrow \kw{OP}.\kw{SPLITROWS}$
                }
            }
            \ElseIf{$|T| \geq 2\beta$ and $|T.\kw{Attributes}| = 1$}{
                $\kw{op} \leftarrow \kw{OP}.\kw{SPLITROWS}$
            }
            \ElseIf{$|T| < 2\beta$ and $|T.\kw{Attributes}| > 1$}{
                $\kw{op} \leftarrow \kw{OP}.\kw{SPLITCOLS}$
            }
            \Return{\kw{op}}
        }
        \Procedure{$\kw{allocBudgetOP}(T, \kw{op}, \epsilon)$}{
            \If{\kw{op} = \kw{OP}.\kw{SPLITCOLS} and $|T.\kw{Attributes}| = 2$}{
                $\epsilon_{p} \leftarrow 0$\;
            }
            \Else{
                $\epsilon_{p} \leftarrow \epsilon/2$\;
            }
       
            \Return{$\epsilon_p, \epsilon - \epsilon_p$}
        }
\end{algorithm}

\begin{align*}
    \sigma(T) = 2\cdot |T.\kw{Attributes}| + \frac{|T|}{\beta} - 2
\end{align*}


\begin{align*}
    \kw{NMI}_{col}  = \big(\frac{2}{|T|}\log(\frac{|T|+1}{2}) + \frac{|T|-1}{|T|}\log(\frac{|T|+1}{|T|-1})\big) / \log(|T|)
\end{align*}

\begin{align*}
    \kw{NMI}_{row}  = & \big(\frac{\log(|T|)}{|T|} - \frac{|T|-1}{|T|}\log(\frac{|T|-1}{|T|})\\ 
    & + \frac{\log(n')}{n'} - \frac{n'-1}{n'}\log(\frac{n'-1}{n'})\big)/(\frac{\log(|T|) + \log(n')}{2})
\end{align*}
where $n'=\max\{|T[\mathcal{S}_L]|, |T[\mathcal{S}_R]|\}$



\clearpage

\begin{algorithm} [ht]
  \caption{Private SPN Construction \kw{PrivSPN} (Beta 4)}
  % \label{alg:SPN}
  \SetKwComment{tcp}{//}{}
  \Input{table $T$, total privacy budget $\epsilon$. } 
  \Output{A tree of SPN $t=(\kw{parent}, \kw{left}, \kw{right})$}
  \SetKwProg{Procedure}{procedure}{}{}
  \Procedure{$\kw{PrivSPN}(T, \epsilon)$}{
    % \tcp*[h]{op is the next splitting operation}\;
    $\kw{op}, \epsilon_\kw{op}, \bar{\epsilon} \leftarrow \kw{planning}(T, \epsilon)$\;
    \If{$\kw{op} = \kw{OP}.\kw{CREATELEAF}$}{
        \Return{\kw{LeafNode}($T, \epsilon_\kw{op}$)}
    }    
    \ElseIf{$\kw{op} = \kw{OP}.\kw{SPLITROWS}$}{
        $(\widetilde{S}_L, \widetilde{S}_R) \leftarrow \kw{splitRowsWithClustering}(T, \epsilon_\kw{op})$\;
        $\kw{parent} \leftarrow \kw{SumNode}(\widetilde{S}_L, \widetilde{S}_R)$\;
        $\epsilon_l \leftarrow \bar{\epsilon}, \epsilon_r \leftarrow \bar{\epsilon}$
    } 
    \ElseIf{$\kw{op} = \kw{OP}.\kw{SPLITCOLS}$}{
        $(\widetilde{S}_L, \widetilde{S}_R) \leftarrow \kw{columnSplit}(T, \epsilon_\kw{op})$\;
        $\kw{parent} \leftarrow \kw{ProductNode}(\widetilde{S}_L, \widetilde{S}_R)$\;
        $\epsilon_l \leftarrow \bar{\epsilon} \cdot \frac{\sigma(T[\widetilde{S}_L])}{\sigma(T[\widetilde{S}_L]) + \sigma(T[\widetilde{S}_R])}, \epsilon_r \leftarrow \bar{\epsilon} - \epsilon_l$
    }
    $\kw{left} \leftarrow \kw{PrivSPN}(T[\widetilde{S}_L], \epsilon_{l})$\;
    $\kw{right} \leftarrow \kw{PrivSPN}(T[\widetilde{S}_R], \epsilon_r)$\;
    \Return{$(\kw{parent}, \kw{left}, \kw{right})$}
    
    % \If{$op = OP.SPLIT\_COLS$}{
    %     $(\textbf{a}_l, \textbf{a}_r, isFail ) \leftarrow split\_cols(T, \textbf{a}, \alpha, force)$\;
    %     $lch \leftarrow splitDatabase(\textbf{a}_l, \textbf{r}, T)$\;
    %     $rch \leftarrow splitDatabase(\textbf{a}_r, \textbf{r}, T)$\;
    %     \Return ProductNode($lch, rch, \textbf{a}, \textbf{r}$)
    % }  
}
\end{algorithm}

\begin{algorithm}
    \caption{Operation Planning \kw{planning} (Beta 4)}
    % \label{alg:plan}
    \Input{table $T$, privacy budget $\epsilon$}
    \Output{next operation $\kw{op}$, privacy budget $\epsilon_\kw{op}$ for $\kw{op}$, remaining privacy budget $\bar{\epsilon}$}
    \KwParam{threshold for column splitting $\alpha$, minimum table size $\beta$, budget ratios $\gamma_1, \gamma_2$}
    \SetKwProg{Procedure}{procedure}{}{}
        \Procedure{$\kw{planning}(T, \epsilon)$}{
            \If{$|T| < 2\beta$ and $|T.\kw{Attributes}| = 1$}{
                $\kw{op} \leftarrow \kw{OP.CREATELEAF}$; $\epsilon_\kw{op} \leftarrow \epsilon$; $\bar{\epsilon}\leftarrow 0$\; 
                \Return\ $\kw{op}, \epsilon_\kw{op}, \bar{\epsilon}$
            }
            % \If{$|T| < 2\beta$ and $|T.\kw{Attributes}| = 2$}{
            %     \Return\ \kw{OP}.\kw{SPLITROWS}, $(0, \frac{\epsilon}{2}, \frac{\epsilon}{2})$
            % }
            $\delta_{col}, \epsilon_\kw{eval} \leftarrow \kw{evalCorr}(T, \epsilon)$\; 
            $\kw{op} \leftarrow \kw{decideOP}(T, \delta_{col})$\;
            $\epsilon_\kw{op} \leftarrow \kw{allocBudgetOP}(T, \kw{op}, \epsilon,  \epsilon_\kw{eval})$\; 
            $\bar{\epsilon} \leftarrow \epsilon - \epsilon_\kw{eval} - \epsilon_\kw{op}$\;
            \Return\ $\kw{op}, \epsilon_\kw{op}, \bar{\epsilon}$
        }
        \Procedure{$\kw{evalCorr}(T, \epsilon)$}{
            \If{$|T| \geq 2\beta$ and $|T.\kw{Attributes}| > 1$}{
                $\epsilon_\kw{eval} \leftarrow \epsilon \cdot \gamma_1$\;
                $(\mathcal{S}_L, \mathcal{S}_R) \leftarrow \kw{columnSplit}(T, \epsilon_\kw{eval} \cdot \gamma_2)$\;
                $\delta_{col} \leftarrow \kw{NMI}_{col}(T[\mathcal{S}_L], T[\mathcal{S}_R]) + \kw{Lap}(\frac{\Delta(\kw{NMI}_{col})}{\epsilon_\kw{eval} \cdot (1-\gamma_2)})$\;
            }
            \Else{
                $\epsilon_\kw{eval} \leftarrow 0$; $\delta_{col} \leftarrow 0$\;
            }
            \Return\ $\delta_{col}, \epsilon_\kw{eval}$
        }
        \Procedure{$\kw{decideOP}(T, \delta_{col})$}{
            \If{$|T| \geq 2\beta$ and $|T.\kw{Attributes}| > 1$}{
                \If{$\delta_{col} \leq \alpha$}{
                    $\kw{op} \leftarrow \kw{OP}.\kw{SPLITCOLS}$
                }
                \Else{
                    $\kw{op} \leftarrow \kw{OP}.\kw{SPLITROWS}$
                }
            }
            \ElseIf{$|T| \geq 2\beta$ and $|T.\kw{Attributes}| = 1$}{
                $\kw{op} \leftarrow \kw{OP}.\kw{SPLITROWS}$
            }
            \ElseIf{$|T| < 2\beta$ and $|T.\kw{Attributes}| > 1$}{
                $\kw{op} \leftarrow \kw{OP}.\kw{SPLITCOLS}$
            }
            \Return{\kw{op}}
        }
        \Procedure{$\kw{allocBudgetOP}(T, \kw{op}, \epsilon, \epsilon_\kw{eval})$}{
            \If{\kw{op} = \kw{OP}.\kw{SPLITCOLS} and $|T.\kw{Attributes}| = 2$}{
                $\epsilon_\kw{op} \leftarrow 0$\;
            }
            \Else{
                $\epsilon_\kw{op} \leftarrow \epsilon/2 - \epsilon_\kw{eval}$\;
            }
       
            \Return{$\epsilon_\kw{op}$}
        }
\end{algorithm}

\begin{align*}
    \sigma(T) = 2^{|T.\kw{Attributes}| + \frac{|T|}{\beta} - 1} + 2^{|T.\kw{Attributes}| + \frac{|T|}{\beta} - 2} - 2
\end{align*}


\begin{align*}
    \kw{NMI}_{col}  = \big(\frac{2}{|T|}\log(\frac{|T|+1}{2}) + \frac{|T|-1}{|T|}\log(\frac{|T|+1}{|T|-1})\big) / \log(|T|)
\end{align*}

\begin{align*}
    \kw{NMI}_{row}  = & \big(\frac{\log(|T|)}{|T|} - \frac{|T|-1}{|T|}\log(\frac{|T|-1}{|T|})\\ 
    & + \frac{\log(n')}{n'} - \frac{n'-1}{n'}\log(\frac{n'-1}{n'})\big)/(\frac{\log(|T|) + \log(n')}{2})
\end{align*}
where $n'=\max\{|T[\mathcal{S}_L]|, |T[\mathcal{S}_R]|\}$

% \clearpage
% \begin{definition}[Laplace mechanism\cite{dwork2014algorithmic}]
%     %(The Laplace Mechanism). 
%     Given any function $F: \mathcal{D} \rightarrow \mathbb{R}^{k}$, the Laplace mechanism is defined as:
%     \begin{align}
%         M_{\mathrm{L}}(D, F(\cdot), \epsilon)=F(D)+\left(N_1, \ldots, N_k\right)
%     \end{align}
%     where $N_i$ are i.i.d. random variables drawn from $Lap(\Delta_{F}/\epsilon)$.
% \end{definition} 

% \begin{definition}[Exponential Mechanism\cite{dwork2014algorithmic}]
%     Let Q be the utility score for choosing the best answer $y$ from the database D. The exponential mechanism $M_{\mathrm{E}}$ samples $y$ with probability proportional to $exp(\frac{\epsilon Q(D,y)}{2\Delta_{Q}})$.
% \end{definition}

\clearpage
\begin{algorithm}[ht]
% \label{alg:privbench}
    \caption{PrivBench (Beta 5)}
    \label{alg:privbench}
    \Input{Database $D$, privacy budget $\epsilon$}
    \Output{Synthetic database $\widehat{D}$}
    \KwParam{Maximum multiplicities $\tau_1,...,\tau_n$.}
    % $\mathcal{O} \leftarrow $ call Algorithm 4 to get generation order\;
    % \For{each private table $T_i$ of $D$}{
    %     $\epsilon_i \leftarrow \frac{\epsilon}{\tau_i \cdot n}$ \;
    % }
    % SPNList $\leftarrow []$\;
    \For{each private table $T_i$ of $D$ }{
        $\epsilon_i \leftarrow \frac{\epsilon \cdot (1-\gamma_f)}{\tau_i \cdot n}$; $t_i \leftarrow \kw{PrivSPN}(T_i, \epsilon_i)$\;
        % SPNList.add($SPN_i$)\;
    }
    % $\epsilon_f \leftarrow $ assign budget for fanout list.\;
    % \For{each pair of tables $(T_i, T_j)$ where $T_i$ refers to $t_j$}{
    %     % $SPN_1, SPN_0 \leftarrow$ SPNs of ($R_1, R_0$)\;
    %     $\mathcal{F}_{i,j} \leftarrow \kw{Fanout}(t_i, t_j)$\;
    % }
    % \For{each SPN $t_i$}{
    %     \small{$\widehat{T}_i \leftarrow \kw{SampleDataFromSPN}(\{t_i\}_{\forall i}, \{\mathcal{F}_{i,j}\}_{\forall i, j})$\;}
    % }
    \For{each SPN $t_i$}{
        \small{$\widehat{T}_i \leftarrow \kw{SampleDataFromSPN}(t_i)$\;}
    }
    \Return $\hat{D}=\set{\hat{T}_1,\dots,\hat{T}_n}$\;
\end{algorithm}


\begin{algorithm}[ht]
% \label{alg:privbench}
    \caption{PrivBench (Beta 6)}
    \label{alg:privbench}
    \Input{Database $D$, privacy budget $\epsilon$}
    \Output{Synthetic database $\widehat{D}$}
    \KwParam{Maximum multiplicities $\tau_1,...,\tau_n$.}
    % $\mathcal{O} \leftarrow $ call Algorithm 4 to get generation order\;
    % \For{each private table $T_i$ of $D$}{
    %     $\epsilon_i \leftarrow \frac{\epsilon}{\tau_i \cdot n}$ \;
    % }
    % SPNList $\leftarrow []$\;
    \For{each private table $T_i$ of $D$ }{
        $\epsilon_i \leftarrow \frac{\epsilon \cdot (1-\gamma_f)}{\tau_i \cdot n}$; $t_i \leftarrow \kw{PrivSPN}(T_i, \epsilon_i)$\;
        % SPNList.add($SPN_i$)\;
    }
    $\epsilon_f \leftarrow $ assign budget for fanout list.\;
    \For{each pair of tables $(T_i, T_j)$ where $T_i$ refers to $t_j$}{
        % $SPN_1, SPN_0 \leftarrow$ SPNs of ($R_1, R_0$)\;
        $\mathcal{F}_{i,j} \leftarrow \kw{PrivFanout}(t_i, t_j)$\;
    }
    \For{each SPN $t_i$}{
        \small{$\widehat{T}_i \leftarrow \kw{SampleDataFromSPN}(\{t_i\}_{\forall i}, \{\mathcal{F}_{i,j}\}_{\forall i, j})$\;}
    }
    % \For{each SPN $t_i$}{
    %     \small{$\widehat{T}_i \leftarrow \kw{SampleDataFromSPN}(t_i)$\;}
    % }
    \Return $\hat{D}=\set{\hat{T}_1,\dots,\hat{T}_n}$\;
\end{algorithm}


\begin{algorithm}[ht]
    \caption{Fanout Table Construction $\kw{PrivFanout}$ (Beta 6)}
    \label{alg:fan}
    \Input{SPNs $t_i, T_j$, privacy budget $\epsilon_f$}
    \Output{Fanout table $\widetilde{\mathcal{F}}_{i,j}$}
    $\mathcal{F}_{i,j} \leftarrow $ empty dictionary \;
    \For{each value $pk$ of the primary key of $T_j$}{
        $\mathcal{F}_{i,j}[pk] \leftarrow$ count the rows in SPN $t_i$ whose value of the foreign key equals $pk$\;
    }
    $\widetilde{\mathcal{F}}_{i,j} \leftarrow \widetilde{\mathcal{F}}_{i,j} + \kw{Lap}(\frac{\tau_{i}}{\epsilon_f})$\;
    \Return $\widetilde{\mathcal{F}}_{i,j}$
\end{algorithm}

\clearpage


\begin{algorithm}[ht]
% \label{alg:privbench}
    \caption{PrivBench (Beta 7)}
    % \label{alg:privbench}
    \Input{Database $D$, privacy budget $\epsilon$}
    \Output{Synthetic database $\widehat{D}$}
    \KwParam{Maximum multiplicities $\tau_1,...,\tau_n$.}
    % $\mathcal{O} \leftarrow $ call Algorithm 4 to get generation order\;
    % \For{each private table $T_i$ of $D$}{
    %     $\epsilon_i \leftarrow \frac{\epsilon}{\tau_i \cdot n}$ \;
    % }
    % SPNList $\leftarrow []$\;
    \For{each private table $T_i$ of $D$ }{
        $\epsilon_i \leftarrow \frac{\epsilon \cdot (1-\gamma_f)}{\tau_i \cdot n}$; $t_i \leftarrow \kw{PrivSPN}(T_i, \epsilon_i)$\;
        % SPNList.add($SPN_i$)\;
    }
    % $\epsilon_f \leftarrow $ assign budget for fanout list.\;
    \For{each pair of tables $(T_i, T_j)$ where $T_i$ refers to $T_j$}{
        % $SPN_1, SPN_0 \leftarrow$ SPNs of ($R_1, R_0$)\;
        $\widetilde{\mathcal{F}}_{i,j} \leftarrow \kw{PrivFanout}(T_i, t_i, PK_{j}, \frac{\epsilon \cdot \gamma_f}{\tau_i \cdot n_\kw{pairs}})$\;
    }
    % \For{each SPN $t_i$}{
    %     \small{$\widehat{T}_i \leftarrow \kw{SampleDataFromSPN}(\{t_i\}_{\forall i}, \{\mathcal{F}_{i,j}\}_{\forall i, j})$\;}
    % }
    \For{each modified SPN $t_i'$}{
        \small{$\widehat{T}_i \leftarrow \kw{SampleDataFromSPN}(t_i')$\;}
    }
    \Return $\hat{D}=\set{\hat{T}_1,\dots,\hat{T}_n}$\;
\end{algorithm}

\begin{algorithm}[ht]
    \caption{Fanout Table Construction $\kw{PrivFanout}$ (Beta 7)}
    % \label{alg:fan}
    \Input{Table $T_i$, SPN $t_i$, primary key $PK_{j}, $privacy budget $\epsilon_f$}
    \Output{Modified SPN $t_i'$}
    Case 1: $\mathcal{A} \leftarrow$ Uniformly sample an attribute of $T_i$\;
    Case 2: $\mathcal{A} \leftarrow$ Find the attribute with the most leaf nodes of $T_i$\;
    Case 3: $\mathcal{A} \leftarrow$ Find the attribute with the least leaf nodes of $T_i$\;
    \For{each leaf node $\kw{leaf}_\mathcal{A}$ of $t_i$ that contains the column of $\mathcal{A}$}{
        Extract subtable $T_i[\mathcal{S}_{\kw{leaf}_\mathcal{A}}]$ from $T_i$ according to the IDs of tuples in $\kw{leaf}_\mathcal{A}$\;
        \For{each value $pk$ of $PK_{j}$}{
            $\mathcal{F}_{i,j}[pk] \leftarrow$ count the rows in $T_i[\mathcal{S}_{\kw{leaf}_\mathcal{A}}]$ whose value of the foreign key equals $pk$\;
        }
        $\widetilde{\mathcal{F}}_{i,j} \leftarrow \mathcal{F}_{i,j} + \kw{Lap}(\frac{\Delta(\mathcal{F}_{i,j})}{\epsilon_f})$\;
        $\kw{leaf}_{FK} \leftarrow \kw{LeafNode}(\widetilde{\mathcal{F}}_{i,j})$\;
        $\kw{parent} \leftarrow \kw{ProdNode}(\mathcal{A}, FK)$\;
        Replace $\kw{leaf}_\mathcal{A}$ in $t_i$ with subtree $(\kw{parent}, \kw{leaf}_\mathcal{A}, \kw{leaf}_{FK})$
    }
    % \For{each value $pk$ of the primary key of $T_j$}{
    %     $\mathcal{F}_{i,j}[pk] \leftarrow$ count the rows in SPN $t_i$ whose value of the foreign key equals $pk$\;
    % }
    % $\widetilde{\mathcal{F}}_{i,j} \leftarrow \widetilde{\mathcal{F}}_{i,j} + \kw{Lap}(\frac{\tau_{i}}{\epsilon_f})$\;
    % \Return $\widetilde{\mathcal{F}}_{i,j}$
\end{algorithm}


\clearpage


\begin{algorithm}[ht]
% \label{alg:privbench}
    \caption{PrivBench (Beta 8)}
    % \label{alg:privbench}
    \Input{Database $D$, privacy budget $\epsilon$}
    \Output{Synthetic database $\widehat{D}$}
    \KwParam{Maximum multiplicities $\tau_1,...,\tau_n$.}
    % $\mathcal{O} \leftarrow $ call Algorithm 4 to get generation order\;
    % \For{each private table $T_i$ of $D$}{
    %     $\epsilon_i \leftarrow \frac{\epsilon}{\tau_i \cdot n}$ \;
    % }
    % SPNList $\leftarrow []$\;
    \For{each private table $T_i$ of $D$ }{
        $\epsilon_i \leftarrow \frac{\epsilon \cdot (1-\gamma_f)}{\tau_i \cdot n}$; $t_i \leftarrow \kw{PrivSPN}(T_i, \epsilon_i)$\;
        % SPNList.add($SPN_i$)\;
    }
    % $\epsilon_f \leftarrow $ assign budget for fanout list.\;
    \For{each pair of tables $(T_i, T_j)$ where $T_i$ refers to $T_j$}{
        % $SPN_1, SPN_0 \leftarrow$ SPNs of ($R_1, R_0$)\;
        $\widetilde{\mathcal{F}}_{i,j} \leftarrow \kw{PrivFanout}(T_i, t_i, PK_{j}, \frac{\epsilon \cdot \gamma_f}{\tau_i \cdot n_\kw{pairs}})$\;
    }
    % \For{each SPN $t_i$}{
    %     \small{$\widehat{T}_i \leftarrow \kw{SampleDataFromSPN}(\{t_i\}_{\forall i}, \{\mathcal{F}_{i,j}\}_{\forall i, j})$\;}
    % }
    \For{each modified SPN $t_i'$}{
        \small{$\widehat{T}_i \leftarrow \kw{SampleDataFromSPN}(t_i')$\;}
    }
    \Return $\hat{D}=\set{\hat{T}_1,\dots,\hat{T}_n}$\;
\end{algorithm}

\begin{algorithm}[ht]
    \caption{Fanout Table Construction $\kw{PrivFanout}$ (Beta 8)}
    % \label{alg:fan}
    \Input{Table $T_i$, SPN $t_i$, primary key $PK_{j}, $privacy budget $\epsilon_f$}
    \Output{Modified SPN $t_i'$}
    Case 1: $\mathcal{A} \leftarrow$ Uniformly sample an attribute of $T_i$\;
    Case 2: $\mathcal{A} \leftarrow$ Find the attribute with the most leaf nodes of $T_i$\;
    Case 3: $\mathcal{A} \leftarrow$ Find the attribute with the least leaf nodes of $T_i$\;
    \For{each leaf node $\kw{leaf}_\mathcal{A}$ of $t_i$ that contains the column of $\mathcal{A}$}{
        Extract subtable $T_i[\mathcal{S}_{\kw{leaf}_\mathcal{A}}]$ from $T_i$ according to the IDs of tuples in $\kw{leaf}_\mathcal{A}$\;
        % \For{each value $pk$ of $PK_{j}$}{
        %     $\mathcal{F}_{i,j}[pk] \leftarrow$ count the rows in $T_i[\mathcal{S}_{\kw{leaf}_\mathcal{A}}]$ whose value of the foreign key equals $pk$\;
        % }
        $\mathcal{F}_{i,j} \leftarrow \kw{hist}(T_i[\mathcal{S}_{\kw{leaf}_\mathcal{A}}], FK)$\;
        $\widetilde{\mathcal{F}}_{i,j} \leftarrow \mathcal{F}_{i,j} + \kw{Lap}(\frac{\Delta(\mathcal{F}_{i,j})}{\epsilon_f})$\;
        $\kw{leaf}_{FK} \leftarrow \kw{LeafNode}(\widetilde{\mathcal{F}}_{i,j})$\;
        $\kw{parent} \leftarrow \kw{ProdNode}(\mathcal{A}, FK)$\;
        Replace $\kw{leaf}_\mathcal{A}$ in $t_i$ with subtree $(\kw{parent}, \kw{leaf}_\mathcal{A}, \kw{leaf}_{FK})$
    }
    % \For{each value $pk$ of the primary key of $T_j$}{
    %     $\mathcal{F}_{i,j}[pk] \leftarrow$ count the rows in SPN $t_i$ whose value of the foreign key equals $pk$\;
    % }
    % $\widetilde{\mathcal{F}}_{i,j} \leftarrow \widetilde{\mathcal{F}}_{i,j} + \kw{Lap}(\frac{\tau_{i}}{\epsilon_f})$\;
    % \Return $\widetilde{\mathcal{F}}_{i,j}$
\end{algorithm}

==> content/analysis-revise.tex <==
\section{Privacy Analysis}
\label{sec:privacy}
In this section, we rigoriously analyze how \ours satisfies DP and how we should allocate privacy budgets to some key steps in \ours.\footnote{All missing proofs can be found in our online appendix: \url{https://drive.google.com/file/d/1mjhKOajBNvN5RbX7k_pvEoFi9DRCWuza/view?usp=sharing}.}

% \subsection{DP Analysis}

% \subsubsection{DP Analysis of \kw{PrivSPN}}
% We first prove that the \kw{Planning}, \kw{ParentGen}, and \kw{ChildrenGen} procedures satisfy DP, and then prove that \kw{PrivSPN} therefore achieves DP.

% \myparagraph{\kw{Planning}}
% The \kw{Planning} procedure consists of the \kw{CorrTrial}, \kw{DecideOP}, and \kw{AllocBudgetOP} subprocedures.
% If the subprocedures satisfy DP, we can conclude that \kw{Planning} ensures DP according to the sequential composition theorem of DP.

% The DP guarantee of \kw{CorrTrial} varies in two cases: (1) When $|T| \geq 2\beta$ and $|T.\kw{Attr}| > 1$, the \kw{CorrTrial} procedure employs the $\epsilon_\kw{eval}\cdot\gamma_2$-differentially private procedure $\kw{ColSplit}(T, \epsilon_\kw{eval}\cdot\gamma_2)$ to compute a perturbed partition $\big(\widehat{\mathcal{S}}_L, \widehat{\mathcal{S}}_R\big)$.
% Then, it calculates the NMI of $(\widehat{\mathcal{S}}_L, \widehat{\mathcal{S}}_R)$ and injects the Laplace noise $\kw{Lap}(\frac{\Delta(\kw{NMI}_{col})}{\epsilon_\kw{eval} \cdot (1-\gamma_2)})$ into it, which ensures $\big(\epsilon_\kw{eval} \cdot (1-\gamma_2)\big)$-DP.
% According to the sequential composition theorem of DP, $\kw{CorrTrial}(T, \epsilon)$ satisfies $\epsilon_\kw{eval}$-DP.
% (2) When $|T| < 2\beta$ or $|T.\kw{Attr}| = 1$, since varying the value of any row in $T$ does not have any impact on the output $(\sigma_{col}, \epsilon_\kw{eval})$, $\kw{CorrTrial}(T, \epsilon)$ satisfies $0$-DP according to Definition \ref{def:dp}.
% Note that we adopt the bounded DP interpretation;
% in the case of unbounded DP, adding/removing a row from $T$ causes the procedure to take the other conditional branch (Lines 11--14), thereby violating DP. 

% Similar to the second case of \kw{CorrTrial}, for both procedures \kw{DecideOP} and \kw{AllocBudgetOP}, because changing the value of any row in $T$ does not affect the table size $|T|$ and the table dimension $|T.\kw{Attr}|$, it also does not impact their outputs.
% Therefore, they ensure $0$-DP. 

% In conclusion, when $|T|<2\beta$ or $|T.\kw{Attr}|=1$, \kw{Planning} satisfies $0$-DP since any change to $T$ does not impact the output (Lines 1--2);
% otherwise, since it sequentially combines \kw{CorrTrial}, \kw{DecideOP}, and \kw{AllocBudgetOP}, $\kw{Planning}(T, \epsilon)$ satisfies the $\epsilon_\kw{eval}$-DP according to the sequential composition theorem of DP, where the value of $\epsilon_\kw{eval}$ differs in different cases (see Lines 12 and 16).
 
% \begin{lemma}
% \label{lem:Planning}
%     For any $\epsilon\geq 0$ and any $\gamma_1 \geq 0$, if $|T| \geq 2\beta$ and $|T.\kw{Attr}| > 1$, $\kw{Planning}(T, \epsilon)$ satisfies $(\epsilon\cdot \gamma_1)$-DP;
%     otherwise, it satisfies $0$-DP.
% \end{lemma}

% \myparagraph{\kw{ParentGen}}
% Then, we show that in any cases of the given operation $\kw{op}$, \kw{ParentGen} achieves DP.
% % \myparagraph{Case 1: $\kw{op} = \kw{OP.LEAF}$}
% (1) When $\kw{op} = \kw{OP.LEAF}$, we ensure DP using the Laplace mechanism.
% That is, we inject Laplacian noise $\kw{Lap}(\frac{\Delta(\kw{hist})}{\epsilon_\kw{op}})$ into the histogram $\kw{hist}(T)$, which satisfies $\epsilon_\kw{op}$-DP.
% % \myparagraph{Case 2: $\kw{op} = \kw{OP.SUM}$} 
% (2) When $\kw{op} = \kw{OP.SUM}$, we employ a differentially private row splitting mechanism $\kw{RowSplit}(T, \epsilon_\kw{op})$ to generate a perturbed row partition $\widetilde{S}_L, \widetilde{S}_R$, which achieves $\epsilon_\kw{op}$-DP.
% % \myparagraph{Case 3: $\kw{op} = \kw{OP.PRODUCT}$}
% (3) When $\kw{op} = \kw{OP.PRODUCT}$, our proposed column splitting mechanism $\kw{ColSplit}(T, \epsilon_\kw{op})$ is essentially an instance of the Exponential mechanism, thereby guaranteeing $\epsilon_\kw{op}$-DP.

% \begin{lemma}
% \label{lem:ParentGen}
%     For any $\kw{op}$ and any $\epsilon_\kw{op} \geq 0$, $\kw{ParentGen}(T,\kw{op},\epsilon_\kw{op})$ satisfies $\epsilon_\kw{op}$-DP.
% \end{lemma}

% \myparagraph{\kw{ChildrenGen}}
% Next, we analyze the DP guarantee of $\kw{ChildrenGen}$ in different cases.
% % \myparagraph{Case 1: $\kw{op} = \kw{OP.LEAF}$}
% (1) When $\kw{op} = \kw{OP.LEAF}$, since \kw{ChildrenGen} always returns two null children, it must satisfy $0$-DP.
% Therefore, in this case, $\kw{PrivSPN(T, \epsilon)}$ achieves $\epsilon$-DP.
% % \myparagraph{Case 2: $\kw{op} = \kw{OP.SUM}$} 
% (2) When $\kw{op} = \kw{OP.SUM}$ or $\kw{op} = \kw{OP.PRODUCT}$, we can prove the DP guarantee by mathematical induction:
% when $\kw{PrivSPN}(T[\widetilde{S}_L], \epsilon_{l})$ (resp. $\kw{PrivSPN}(T[\widetilde{S}_R], \epsilon_r)$) returns a subtree with only a leaf node, as shown in case 1, it satisfies $\epsilon_l$-DP (resp. $\epsilon_r$-DP);
% otherwise, assuming $\kw{PrivSPN}(T[\widetilde{S}_L], \epsilon_{l})$ (resp. $\kw{PrivSPN}(T[\widetilde{S}_R], \epsilon_r)$) satisfies $\epsilon_l$-DP (resp. $\epsilon_r$-DP), we conclude that $\kw{ChildrenGen}(T, \kw{op}, \bar{\epsilon})$ satisfies $\bar{\epsilon}$-DP according to the sequential composition theorem, where $\bar{\epsilon} = \epsilon_l + \epsilon_r$.
% % \myparagraph{Case 3: $\kw{op} = \kw{OP.PRODUCT}$}
% % The proof for Case 3 follows the same logic as that for Case 2.
% Note that varying any row of $T$ does not affect $\sigma(T[\widetilde{S}_L])$ and $\sigma(T[\widetilde{S}_R])$ since they are functions of a table's size and dimension.


% \begin{lemma}
% \label{lem:ChildrenGen}
%     For any $\bar{\epsilon} \geq 0$, if $\kw{op} = \kw{OP.LEAF}$, $\kw{ChildrenGen}(T, \kw{op}, \bar{\epsilon})$ satisfies $0$-DP;
%     otherwise, it satisfies $\bar{\epsilon}$-DP.
% \end{lemma}

% \myparagraph{\kw{PrivSPN}}
% Based on Lemmas \ref{lem:Planning}, \ref{lem:ParentGen}, and \ref{lem:ChildrenGen}, we derive the following theorem through sequential composition.

% \begin{lemma}
%     For any $\epsilon \geq 0$, $\kw{PrivSPN}(T, \epsilon)$ satisfies $\epsilon$-DP.
% \end{lemma}


% \subsubsection{DP Analysis of \kw{PrivFanout}}
% \kw{PrivFanout} achieves DP because we inject the Laplace noise into the fanout table in Line 5, which implements the differentially private Laplace mechanism.

% \begin{lemma}
%     For any SPN $t_i$, any primary key $PK_j$, and any $\epsilon \geq 0$, $\kw{PrivFanout}(T_i, t_i, PK_j, \epsilon)$ satisfies $\epsilon$-DP.
% \end{lemma}






\subsection{Privacy Analysis on \kw{PrivSPN}}
\label{sec:dp:privspn}
In this subsection, we first prove that the \kw{Planning}, \kw{ParentGen}, and \kw{ChildrenGen} procedures satisfy DP, and then prove that \kw{PrivSPN} therefore achieves DP.

\subsubsection{Analysis of \kw{Planning}}
The \kw{Planning} procedure consists of the \kw{CorrTrial}, \kw{DecideOP}, and \kw{AllocBudgetOP} subprocedures.
If the subprocedures satisfy DP, we can conclude that \kw{Planning} ensures DP according to the sequential composition theorem of DP~\cite{dwork2006differential}.

% \myparagraph{Procedure \kw{ColSplit}}
% As shown in Algorithm \ref{alg:SPN}, the \kw{ColSplit} procedure employs the Exponential mechanism to sample a column partition, which ensures DP.

% \begin{lemma}
%     For any $\epsilon\geq 0$, Procedure $\kw{ColSplit}(T, \epsilon)$ in Algorithm \ref{alg:colsplit} satisfies $\epsilon$-DP.
% \end{lemma}

\myparagraph{\kw{CorrTrial}}
(1) When $|T| \geq 2\beta$ and $|T.\kw{Attr}| > 1$, the \kw{CorrTrial} procedure employs the $\epsilon_\kw{eval}\cdot\gamma_2$-DP procedure $\kw{ColSplit}(T, \epsilon_\kw{eval}\cdot\gamma_2)$ to compute a perturbed partition $\big(\widehat{\mathcal{S}}_L, \widehat{\mathcal{S}}_R\big)$.
Then, it calculates the NMI of $(\widehat{\mathcal{S}}_L, \widehat{\mathcal{S}}_R)$ and injects the Laplace noise $\kw{Lap}(\frac{\Delta(\kw{NMI}_{col})}{\epsilon_\kw{eval} \cdot (1-\gamma_2)})$ into it, which ensures $\big(\epsilon_\kw{eval} \cdot (1-\gamma_2)\big)$-DP.
Consequently, according to the sequential composition theorem of DP~\cite{dwork2006differential}, $\kw{CorrTrial}(T, \epsilon)$ satisfies $\epsilon_\kw{eval}$-DP.
(2) When $|T| < 2\beta$ or $|T.\kw{Attr}| = 1$, since varying the value of any row in $T$ does not have any impact on the output $(\sigma_{col}, \epsilon_\kw{eval})$, $\kw{CorrTrial}(T, \epsilon)$ satisfies $0$-DP according to Definition \ref{def:dp}.
Note that we adopt the bounded DP interpretation;
in the case of unbounded DP, adding/removing a row from $T$ causes the procedure to take the other conditional branch (i.e., Lines 11--14), thereby breaking the DP guarantee. 

% \begin{lemma}
%     For any $\epsilon\geq 0$, if $|T| \geq 2\beta$ and $|T.\kw{Attr}| > 1$, $\kw{CorrTrial}(T, \epsilon)$ satisfies $\epsilon_\kw{eval}$-DP;
%     otherwise, it satisfies $0$-DP.
% \end{lemma}

\myparagraph{\kw{DecideOP} and \kw{AllocBudgetOP}}
Similar to the second case of \kw{CorrTrial}, for both procedures \kw{DecideOP} and \kw{AllocBudgetOP}, because changing the value of any row in $T$ does not affect the table size $|T|$ and the table dimension $|T.\kw{Attr}|$, it also does not impact their outputs.
Therefore, they ensure $0$-DP. 

% \begin{lemma}
%     For any $\sigma_{col}\in \mathbb{R}$, $\kw{DecideOP}(T, \sigma_{col})$ satisfies $0$-DP.
% \end{lemma}

% \begin{lemma}
%     For any $\kw{op}$, any $\epsilon \geq 0$, and any $\epsilon_\kw{eval} \geq 0$, procedure $\kw{allocBudget}(T, \kw{op}, \epsilon, \epsilon_\kw{eval})$ satisfies $0$-DP.
% \end{lemma}

\myparagraph{\kw{Planning}}
When $|T|<2\beta$ or $|T.\kw{Attr}|=1$, \kw{Planning} satisfies $0$-DP since any change to $T$ does not impact the output (Lines 1--2);
otherwise, since it sequentially combines \kw{CorrTrial}, \kw{DecideOP}, and \kw{AllocBudgetOP}, $\kw{Planning}(T, \epsilon)$ satisfies the $\epsilon_\kw{eval}$-DP according to the sequential composition theorem of DP~\cite{dwork2006differential}, where the value of $\epsilon_\kw{eval}$ differs in different cases (see Lines 12 and 16).
 
\begin{lemma}
\label{lem:Planning}
    For any $\epsilon\geq 0$ and any $\gamma_1 \geq 0$, if $|T| \geq 2\beta$ and $|T.\kw{Attr}| > 1$, $\kw{Planning}(T, \epsilon)$ satisfies $(\epsilon\cdot \gamma_1)$-DP;
    otherwise, it satisfies $0$-DP at the table level.
\end{lemma}


\subsubsection{Analysis of \kw{ParentGen}}
Then, we show that in any cases of the given operation $\kw{op}$, \kw{ParentGen} achieves DP.
% \myparagraph{Case 1: $\kw{op} = \kw{OP.LEAF}$}
(1) When $\kw{op} = \kw{OP.LEAF}$, we ensure DP using the Laplace mechanism.
That is, we inject Laplacian noise $\kw{Lap}(\frac{\Delta(\kw{hist})}{\epsilon_\kw{op}})$ into the histogram $\kw{hist}(T)$, which satisfies $\epsilon_\kw{op}$-DP.
% \myparagraph{Case 2: $\kw{op} = \kw{OP.SUM}$} 
(2) When $\kw{op} = \kw{OP.SUM}$, we employ a DP row splitting mechanism $\kw{RowSplit}(T, \epsilon_\kw{op})$ to generate a perturbed row partition $\widetilde{S}_L, \widetilde{S}_R$, which achieves $\epsilon_\kw{op}$-DP.
% \myparagraph{Case 3: $\kw{op} = \kw{OP.PRODUCT}$}
(3) When $\kw{op} = \kw{OP.PRODUCT}$, our column splitting mechanism $\kw{ColSplit}(T, \epsilon_\kw{op})$ is essentially an instance of the Exponential mechanism, thereby guaranteeing $\epsilon_\kw{op}$-DP.

\begin{lemma}
\label{lem:ParentGen}
    For any $\kw{op}$ and any $\epsilon_\kw{op} \geq 0$, $\kw{ParentGen}(T,\kw{op},\epsilon_\kw{op})$ satisfies $\epsilon_\kw{op}$-DP at the table level.
\end{lemma}

\subsubsection{Analysis of \kw{ChildrenGen}}
Next, we analyze the DP guarantee of $\kw{ChildrenGen}$ in different cases.
% \myparagraph{Case 1: $\kw{op} = \kw{OP.LEAF}$}
(1) When $\kw{op} = \kw{OP.LEAF}$, since \kw{ChildrenGen} always returns two null children, it must satisfy $0$-DP.
Therefore, in this case, $\kw{PrivSPN(T, \epsilon)}$ achieves $\epsilon$-DP.
% \myparagraph{Case 2: $\kw{op} = \kw{OP.SUM}$} 
(2) When $\kw{op} = \kw{OP.SUM}$, Theorem \ref{thm:sumnode} shows that in the case of row splitting, the privacy budgets for constructing the tree $(\kw{parent}, \kw{left}, \kw{right})$ satisfies a parallel composition property:
$$\epsilon = \epsilon_\kw{eval} + \epsilon_\kw{op} + \max\{\epsilon_l, \epsilon_r\} = \epsilon_\kw{eval} + \epsilon_\kw{op} + \bar{\epsilon}.$$
Therefore, to optimize the utility of the subtrees, we maximize each subtree's privacy budget and set $\epsilon_l = \epsilon_r = \bar{\epsilon}$.
Note that Theorem \ref{thm:sumnode} differs from the celebrated parallel composition theorem \cite{dwork2006differential}:
their theorem assumes unbounded DP while our theorem considers bounded DP.
% their theorem assumes unbounded DP and a deterministic function for row splitting, while our theorem considers bounded DP and requires that the row partition is given.
(3) When $\kw{op} = \kw{OP.PRODUCT}$, we allocate privacy budgets based on the scales of the subtrees (Line 18).
Intuitively, a subtree with a larger scale should be assigned with a larger privacy budget to balance their utility.
Thus, their privacy budgets $\epsilon_l, \epsilon_r$ are proportional to their scales $\sigma(T[\widetilde{S}_L]), \sigma(T[\widetilde{S}_R])$.
The scale metric $\sigma$ is a function of the given table's size and dimension, which will be defined in Theorem \ref{thm:down-top} based on our privacy analysis.

\begin{theorem}[Parallel composition under bounded DP]
\label{thm:sumnode}
    % Consider $K$ algorithms $\mathcal{M}_1,\dots,\mathcal{M}_K$ that satisfy $\epsilon_1$-DP,...,$\epsilon_K$-DP, respectively.
    Given a row partition $(\mathcal{S}_1,\dots, \mathcal{S}_K)$, publishing $\mathcal{M}_1(T[\mathcal{S}_1]),\dots,\mathcal{M}_K(T[\mathcal{S}_K])$ satisfies $\max\set{\epsilon_1,\dots, \epsilon_K}$-DP at the database level, where $\mathcal{S}_k$ is a subset of row indices and $\mathcal{M}_k$ is a table-level $\epsilon_k$-DP algorithm, $\forall k \in [K]$.
\end{theorem}

% \begin{theorem}
% \label{thm:sumnode}
%     When the root node of a subtree $T_0$ is a sum node, the privacy budget required to construct this tree $\epsilon_0 = \epsilon_r + \max\{\epsilon_1, \epsilon_2\}$, where $\epsilon_1$ is the privacy budget consumed to construct the left subtree of $T_0$, and $\epsilon_2$ is the privacy cost of the right subtree.
% \end{theorem}

Consequently, when $\kw{op} = \kw{OP.SUM}$ or $\kw{op} = \kw{OP.PRODUCT}$, we can prove the DP guarantee by mathematical induction:
when $\kw{PrivSPN}(T[\widetilde{S}_L], \epsilon_{l})$ (resp. $\kw{PrivSPN}(T[\widetilde{S}_R], \epsilon_r)$) returns a subtree with only a leaf node, as shown in case 1, it satisfies $\epsilon_l$-DP (resp. $\epsilon_r$-DP);
otherwise, assuming $\kw{PrivSPN}(T[\widetilde{S}_L], \epsilon_{l})$ (resp. $\kw{PrivSPN}(T[\widetilde{S}_R], \epsilon_r)$) satisfies $\epsilon_l$-DP (resp. $\epsilon_r$-DP), we conclude that $\kw{ChildrenGen}(T, \kw{op}, \bar{\epsilon})$ satisfies $\bar{\epsilon}$-DP according to the sequential composition theorem~\cite{dwork2006differential} or Theorem \ref{thm:sumnode}, where $\bar{\epsilon} = \epsilon_l + \epsilon_r$ or $\bar{\epsilon} = \max\{\epsilon_l, \epsilon_r\}$.
% \myparagraph{Case 3: $\kw{op} = \kw{OP.PRODUCT}$}
% The proof for Case 3 follows the same logic as that for Case 2.
Note that varying any row of $T$ does not affect $\sigma(T[\widetilde{S}_L])$ and $\sigma(T[\widetilde{S}_R])$ since they are functions of a table's size and dimension.


\begin{lemma}
\label{lem:ChildrenGen}
    For any $\bar{\epsilon} \geq 0$, if $\kw{op} = \kw{OP.LEAF}$, $\kw{ChildrenGen}(T, \kw{op}, \widetilde{\mathcal{S}}_L, \widetilde{\mathcal{S}}_R, \bar{\epsilon})$ satisfies table-level $0$-DP;
    otherwise, it satisfies table-level $\bar{\epsilon}$-DP.
\end{lemma}

\subsubsection{Analysis of \kw{PrivSPN}}
Based on Lemmas \ref{lem:Planning}, \ref{lem:ParentGen}, and \ref{lem:ChildrenGen}, we conclude the DP gurantee of \kw{PrivSPN} through sequential composition.

\begin{lemma}
    For any $\epsilon \geq 0$, $\kw{PrivSPN}(T, \epsilon)$ satisfies table-level $\epsilon$-DP.
\end{lemma}

In addition, since \kw{PrivSPN} allocates the privacy budget $\epsilon$ from the root to the leaf nodes in a top-down manner, it may result in insufficient budgets allocated to the leaf nodes.
Consequently, an interesting question arises: If we allocate a privacy budget $\epsilon_\kw{leaf}$ to all leaf nodes, how large the total privacy budget $\epsilon$ should be?
Theorem \ref{thm:down-top} answers the question and instructs the design of the scale metirc.
That is, if we guarantee a privacy budget $\epsilon_\kw{leaf}$ for each leaf node, then constructing the $\kw{left}$ and $\kw{right}$ subtrees should satisfy $\sigma(T[\widetilde{S}_L])$-DP and $\sigma(T[\widetilde{S}_R])$-DP, respectively.
Therefore, the privacy budgets $\epsilon_l, \epsilon_r$ should be proportional to the corresponding scales (see Line 17 of Algorithm \ref{alg:SPN}).
In our experiments, we set the scale metric as defined in Theorem \ref{thm:down-top} for \kw{PrivSPN}.

\begin{theorem}
  \label{thm:down-top}
    Let $\mathcal{T}$ denote the set of all possibles subtables of $T$ with $|t| < 2\beta$ and $t.\kw{Attr}=1$, $\forall t \in \mathcal{T}$.
    If for any $t\in \mathcal{T}$, $\kw{PrivSPN}(T, \epsilon)$ calls $\kw{PrivSPN}(t, \epsilon_\kw{leaf})$, $\kw{PrivSPN}(T, \epsilon)$ satisfies table-level $\epsilon$-DP, where $\sigma(T)=2^{|T.\kw{Attr}| + \frac{|T|}{\beta} - 2}\cdot |T.\kw{Attr}| \cdot \frac{|T|}{\beta}$.  
\end{theorem}

\subsection{Privacy Analysis on \kw{PrivFanout}}
For each leaf node $\kw{leaf}_{FK}$, \kw{PrivFanout} injects the Laplace noise into the fanout table $\mathcal{F}_{i,j}$ (Line 5), which implements the $\epsilon$-differentially private Laplace mechanism.
Then, according to Theorem \ref{thm:sumnode}, publishing all the leaf nodes $\kw{leaf}_{FK}$ with perturbed fanout tables also satisfies $\epsilon$-DP due to the nature of parallel composition.
Therefore, \kw{PrivFanout} ensures DP.

\begin{lemma}
    For any SPN $t_i$, any primary key $PK_j$, and any $\epsilon \geq 0$, $\kw{PrivFanout}(T_i, t_i, PK_j, \epsilon)$ satisfies $\epsilon$-DP at the table level.
\end{lemma}

\subsection{Privacy Analysis on \ours}
\label{sec:analysis_privbench}
% Then, given that both \kw{PrivSPN} and \kw{PrivFanout} satisfy DP, the DP guarantee of the \ours algorithm is established according to the sequential composition theorem of DP.

% Given that the \kw{PrivSPN} algorithm ensures DP, the \ours algorithm obviously satisfies DP according to the postprocessing theorem of DP.
% Intuitively, both the \kw{CalcFanout} and \kw{SampleDataFromSPNs} procedures do not require any raw tables as input and process perturbed SPNs, which does not compromise DP.




Given that both \kw{PrivSPN} and \kw{PrivFanout} satisfy DP, the DP guarantee of the \ours algorithm is established according to Theorem \ref{thm:table-to-db-dp}.
Note that to measure the indistinguishability level of database-level DP, we cannot simply accumulate the privacy budgets $\epsilon_i$ assigned to each private table $T_i \in D$ for table-level DP, i.e., $\epsilon \neq \sum_{i \in [n]} \epsilon_i$.
Intuitively, while table-level DP only guarantees the indistinguishability of neighboring tables, database-level DP requires indistinguishability of two tables that differ in at most $\tau_i$ tuples because those tuples may depend on a single tuple in the primary private table.
Consequently, as shown in Corollary \ref{coro:privbench}, the indistinguishability levels of procedures $\kw{PrivSPN}$ and $\kw{PrivFanout}$ at the table level should be reduced by factor $\tau_i$ for database-level DP.
Therefore, to ensure $\epsilon$-DP for \ours, we can allocate the given privacy budget $\epsilon$ as follows: $$\epsilon^s_i=\frac{\epsilon \cdot (1-\gamma)}{\tau_i \cdot n}, \quad \epsilon^f_i=\frac{\epsilon \cdot \gamma}{\tau_i \cdot n_\kw{pairs}},$$
where $\gamma\in[0,1]$ is the ratio of privacy budget allocated for fanout construction and $n_\kw{pairs}$ is the number of all referential pairs $(T_i, T_j)$.
In our experiments, we follow the above setting of privacy budgets $\epsilon^s_i, \epsilon^s_f$ for \ours.

% That is, the $\ours(D, \epsilon)$ algorithm that consists of procedures $\kw{PrivSPN}(T_i, \frac{\epsilon \cdot (1-\gamma_f)}{\tau_i \cdot n})$ and $\kw{PrivSPN}(T_i, \frac{\epsilon \cdot \gamma_f}{\tau_i \cdot n_\kw{pairs}})$ satisfies $\epsilon$-DP because $$\epsilon = \sum_{i\in[T]} \frac{\epsilon \cdot (1-\gamma_f)}{\tau_i \cdot n} \cdot \tau_i + \sum_{T_i \text{ refers to } T_j} \frac{\epsilon \cdot \gamma_f}{\tau_i \cdot n_\kw{pairs}} \cdot \tau_i.$$


\begin{theorem}
\label{thm:table-to-db-dp}
    Given $\mathcal{M}_i$ that satisfies $\epsilon_i$-DP at the table level for all $i\in[n]$, $\mathcal{M}(D)=\big(\mathcal{M}_1(T_1),...,\mathcal{M}_n(T_n)\big)$ satisfies $\sum_{i\in[n]}\tau_i\cdot\epsilon_i$-DP at the database level, where $\tau_i$ is the maximum multiplicity of $T_i$.
\end{theorem}

\begin{corollary}[of Theorem \ref{thm:table-to-db-dp}]
\label{coro:privbench}
    \ours satisfies $(\sum_{i\in[n]}\tau_i\cdot\epsilon^s_i+\sum_{T_i \text{ refers to } T_j} \tau_i\cdot\epsilon^f_i)$-DP at the database level.
\end{corollary}



==> content/overview-revise.tex <==
\section{Solution Overview}
\label{sec:overview}
In this section, we provide an overview of \ours. 

% \begin{figure}
%   \centering
%   \includegraphics[width=\linewidth]{figure/SPN_flow_chart.pdf}
%   \caption{Algorithm workflow for constructing an SPN (Sum-Product Network).}
%   \label{fig:SPNflowchart}
% \end{figure}

We propose utilizing Sum-Product Networks (SPNs) to address the two concerns outlined in Section~\ref{sec:preliminaries}. SPNs, due to their excellent performance in representing complex dependencies and data distributions at multiple granularities, have been employed in cardinality estimation~\cite{DeepDB}, a prevalent approach intrinsically connected to estimating the runtime cost of queries. Drawing inspiration from this, we adapt the output in \cite{DeepDB} to produce a synthesized database, designed to closely resemble the input database in terms of data distribution and cardinality upon query execution.

Our proposed solution involves a two-phase process for database synthesis. In the first phase, we partition the input database. In particular, we construct SPNs on relation tables of the input database instance $D$ through recursive partitioning, assigning one SPN per relation. A histogram is built for each leaf node of the SPNs. Furthermore, we join the nodes of primary keys (PK) and foreign keys (FK) that adhere to reference constraints, utilizing a Private Fanout Table. The SPNs of $D$, conjoined through the PK-FK nodes, form a Multi-SPN. Notably, this phase is privacy-preserving; noise is added at each procedural step to ensure the overall algorithm complies with differential privacy principles. In the second phase, we sample from the SPN leaf nodes, conduct post-processing, and stitch the samples along SPN paths to fabricate the synthetic database instance $D'$. Since the first phase has already ensured differential privacy, this phase does not need to inject privacy preservation. 

% Solution to Concern \#1: 
% We propose constructing SPNs over relational tables, which is equivalent to row and column partitioning. Row partitioning preserves tuple similarity. Column partitioning uses attribute correlations. Together, they enable fine-grained data splits. After injecting noise and sampling within each split, the SPN stitches data blocks back to original size, maintaining correlations and similarities to preserve distributions. By performing data synthesis within SPN partitions under differential privacy, we can capture broad distributional characteristics. 

% Solution to Concern \#2: 
% The column partitioning of SPNs based on attribute correlation can adaptively determine split points to maximally preserve dependencies. This reduces cardinality errors for queries. Building on SPNs, we propose Multi-SPNs to handle multi-table synthesis, connecting SPN nodes across tables using FK-PK constraints. For multi-table data, linking SPNs using schema constraints enables smoothly propagating keys and tuples across tables during the stage of generation. This avoids the need for separate key allocation procedures that may discard learned dependencies. Our solution leverages the relational inductive biases provided by SPNs to improve multi-table cardinality preservation under differential privacy. Experiments show our approach provides lower cardinality errors compared to alternatives. 



==> savespace.tex <==
\usepackage[all=normal, floats, bibnotes, wordspacing, charwidths, indent, lists]{savetrees}

\makeatletter%
%
\skip\footins 8.1pt plus 4pt minus 2pt % Space between last line of text top
                                      % and of first footnote.
\floatsep 5pt plus 2pt minus 2pt        % Space between adjacent floats moved
                                         % to top or bottom of text page.
\textfloatsep 5pt plus 2pt minus 4pt    % Space between main text and floats
                                         % at top or bottom of page.
\intextsep 5pt plus 2pt minus 2pt       % Space between in-text figures and
                                         % text.
%\@maxsep 5pt                            % The maximum of \floatsep,
                                         % \textfloatsep and \intextsep (minus
                                         % the stretch and shrink).
\dblfloatsep 5pt plus 0pt minus 0pt     % Same as \floatsep for double-column
                                         % figures in two-column mode.
\dbltextfloatsep 5pt plus 0pt minus 0pt % \textfloatsep for double-column
                                         % floats.
%\@dblmaxsep 5pt                         % The maximum of \dblfloatsep and
                                         % \dbltexfloatsep.
